Geometric properties of the golden ration Thompson's group

We show that all three golden ratio Thompson's groups $F_\tau$, $T_\tau$ and $V_\tau$ embed in the asynchronous rational group. We prove properties of the Cayley graph of the monoid $M = \langle L, R : LR^2 = RL^2 \rangle$, whose topological full group is $V_\tau$. In particular, we compute a distance function for the Cayley graph of the monoid $M$. Additionally, we prove that this Cayley graph is hyperbolic in the sense of Gromov. Our analysis reveals that the horofunction boundary of this graph is homeomorphic to a space resembling a Cantor-like set, with additional isolated points situated between each pair of breakpoints.

==> Background_section/figure_code.tex <==
\begin{figure}
\centering
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2
        [,l*=2,edge label={node[end,left]{$[0,\tau^4]$}}]
        [,edge label={node[end,right]{$[\tau^2,1]$}}]
    ]
    [,edge label={node[end,right]{$[\tau^4,\tau^2]$}}]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$[0,\tau^2]$}}]
    [
        [,l*=2,edge label={node[end,left]{$[\tau^2,\tau]$}}]
        [,edge label={node[end,right]{$[\tau^2,1]$}}]
    ]
]
\end{forest}

\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$[0,\tau^2]$}}]
    [
        [,l*=2
            [,l*=2,edge label={node[end,left]{$[\tau^2,\tau^2+\tau^5]$}}]
            [,edge label={node[end,right]{$[\tau,1]$}}]
        ]
        [,edge label={node[end,right]{$[\tau^2+\tau^5,\tau]$}}]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$[0,\tau^2]$}}]
    [
        [,l*=2,edge label={node[end,left]{$[\tau^2,\tau]$}}]
        [
            [,l*=2,edge label={node[end,left]{$[\tau,\tau+\tau^4]$}}]
            [,edge label={node[end,right]{$[\tau+\tau^4,1]$}}]
        ]
    ]
]
\end{forest}
    \caption{The generators $x_0$ and $x_1$ as tree diagrams.}
    \label{fig:x_n gen1}
\end{figure}

\begin{figure}
\centering
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2
        [,edge label={node[end,left]{$[0,\tau^4]$}}]
        [,l*=2,edge label={node[end,right]{$[\tau^2,1]$}}]
    ]
    [,edge label={node[end,right]{$[\tau^4,\tau^2]$}}]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$[0,\tau^2]$}}]
    [
        [,l*=2,edge label={node[end,left]{$[\tau^2,\tau]$}}]
        [,edge label={node[end,right]{$[\tau^2,1]$}}]
    ]
]
\end{forest}

\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$[0,\tau^2]$}}]
    [
        [,l*=2
            [,edge label={node[end,left]{$[\tau^2,\tau^2+\tau^4]$}}]
            [,l*=2,edge label={node[end,right]{$[\tau,1]$}}]
        ]
        [,edge label={node[end,right]{$[\tau^2+\tau^4,\tau]$}}]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$[0,\tau^2]$}}]
    [
        [,l*=2,edge label={node[end,left]{$[\tau^2,\tau]$}}]
        [
            [,l*=2,edge label={node[end,left]{$[\tau,\tau+\tau^4]$}}]
            [,edge label={node[end,right]{$[\tau+\tau^4,1]$}}]
        ]
    ]
]
\end{forest}
    \caption{The generators $y_0$ and $y_1$ as tree diagrams.}
    \label{fig:y_n gen1}
\end{figure}

\begin{figure}
\centering
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$a$}}]
    [
        [,l*=2,edge label={node[end,left]{$b$}}]
        [,edge label={node[end,right]{$c$}}]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$c$}}]
    [
        [,l*=2,edge label={node[end,left]{$a$}}]
        [,edge label={node[end,right]{$b$}}]
    ]
]
\end{forest}

\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[   [,l*=2,edge label={node[end,left]{$a$}}]
    [
        [,l*=2,edge label={node[end,left]{$b$}}]
        [
            [,l*=2,edge label={node[end,left]{$c$}}]
            [,edge label={node[end,right]{$d$}}]
        ]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[   [,l*=2,edge label={node[end,left]{$d$}}]
    [
        [,l*=2,edge label={node[end,left]{$a$}}]
        [
            [,l*=2,edge label={node[end,left]{$b$}}]
            [,edge label={node[end,right]{$c$}}]
        ]
    ]
]
\end{forest}
    \caption{The generators $c_1$ and $c_2$ as tree diagrams. The labels on the leaves determine which domain intervals map to which range intervals.}
    \label{fig:c_1 c2 gen}
\end{figure}

\begin{figure} 
\centering
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$a$}}]
    [
        [,l*=2,edge label={node[end,left]{$b$}}]
        [,edge label={node[end,right]{$c$}}]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[end,left]{$b$}}]
    [
        [,l*=2,edge label={node[end,left]{$a$}}]
        [,edge label={node[end,right]{$c$}}]
    ]
]
\end{forest}

\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[   [,l*=2,edge label={node[end,left]{$a$}}]
    [
        [,l*=2,edge label={node[end,left]{$b$}}]
        [
            [,l*=2,edge label={node[end,left]{$c$}}]
            [,edge label={node[end,right]{$d$}}]
        ]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[   [,l*=2,edge label={node[end,left]{$a$}}]
    [
        [,l*=2,edge label={node[end,left]{$c$}}]
        [
            [,l*=2,edge label={node[end,left]{$b$}}]
            [,edge label={node[end,right]{$d$}}]
        ]
    ]
]
\end{forest}
    \caption{The generators $\pi_0$ and $\pi_1$ as tree diagrams.}
    \label{fig:pi_0 pi_1 gen}
\end{figure}

\begin{figure}
\[
\begin{tikzpicture}[scale=0.35]
\draw (0,6) node[anchor=north]{}
-- (-6, 2) node[anchor=south]{}
-- (-4,-5) node[anchor=north]{}
-- (4,-5) node[anchor=north]{}
-- (6,2) node[anchor=north]{}
--cycle;

\draw (0,-4) node[anchor=north]{}
-- (-4,-1) node[anchor=south]{}
-- (-2,3) node[anchor=north]{}
-- (2,3) node[anchor=north]{}
-- (4,-1) node[anchor=north]{}
--cycle;



\draw (-2,3) node[anchor=north]{}
--(0,6) node[anchor=north]{}
-- (2,3) node[anchor=north]{};

\draw (-4,-1) node[anchor=south]{}
--(-6, 2) node[anchor=south]{}
-- (-2,3) node[anchor=north]{};

\draw (0,-4) node[anchor=north]{}
-- (-4,-5) node[anchor=north]{}
-- (-4,-1) node[anchor=south]{};

\draw(0,-4) node[anchor=north]{}
--  (4,-5) node[anchor=north]{}
--(4,-1) node[anchor=north]{};

\draw (2,3) node[anchor=north]{}
-- (6,2) node[anchor=north]{}
-- (4,-1) node[anchor=north]{};

\draw (0,-4) node[anchor=north]{}
--(0,0) node[anchor=north]{};

\draw (-4,-1) node[anchor=south]{}
--(0,0) node[anchor=north]{};

\draw (-2,3) node[anchor=north]{}
--(0,0) node[anchor=north]{};

\draw (2,3) node[anchor=north]{}
--(0,0) node[anchor=north]{};

\draw (4,-1) node[anchor=north]{}
--(0,0) node[anchor=north]{};


\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (6,2) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (4,-5) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-4,-5) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-6, 2) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (0,6) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (0,-4) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-4,-1) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-2,3) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (2,3) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (4,-1) {};
\node[circle,fill=red,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (0,0) {};

\draw(0, 0.2) node[anchor=south]{$x$};

\end{tikzpicture}
\]
\end{figure}

\begin{figure}
\[
\begin{tikzpicture}[scale=0.35]
\draw (0,6) node[anchor=north]{}
-- (-6, 2) node[anchor=south]{}
-- (-4,-5) node[anchor=north]{}
-- (4,-5) node[anchor=north]{}
-- (6,2) node[anchor=north]{}
--cycle;

\draw (0,-4) node[anchor=north]{}
-- (-4,-1) node[anchor=south]{}
-- (-2,3) node[anchor=north]{}
-- (2,3) node[anchor=north]{}
-- (4,-1) node[anchor=north]{}
--cycle;






\draw[-{Stealth[length=3mm]}](0,6) node[anchor=north]{}
-- (1,4.5) node[anchor=north]{};
\draw(1,4.5) node[anchor=north]{}
-- (2,3) node[anchor=north]{};

\draw[-{Stealth[length=3mm]}](0,6) node[anchor=north]{}
-- (-1,4.5) node[anchor=north]{};
\draw(-1,4.5) node[anchor=north]{}
-- (-2,3) node[anchor=north]{};

\draw[-{Stealth[length=3mm]}] (-6, 2) node[anchor=south]{}
-- (-4,2.5) node[anchor=north]{};
\draw (-4, 2.5) node[anchor=south]{}
-- (-2,3) node[anchor=north]{};

\draw[-{Stealth[length=3mm]}] (-6, 2) node[anchor=south]{}
-- (-5,0.5) node[anchor=south]{};
\draw(-5, 0.5) node[anchor=south]{}
-- (-4,-1) node[anchor=south]{};

\draw[-{Stealth[length=3mm]}](-4,-5) node[anchor=north]{}
-- (-4,-3) node[anchor=south]{};
\draw(-4,-3) node[anchor=north]{}
-- (-4,-1) node[anchor=south]{};

\draw[-{Stealth[length=3mm]}](-4,-5) node[anchor=north]{}
-- (-2,-4.5) node[anchor=north]{}; 
\draw(-2,-4.5) node[anchor=north]{}
-- (0,-4) node[anchor=north]{}; 

\draw[-{Stealth[length=3mm]}](4,-5) node[anchor=north]{}
--(4,-3) node[anchor=north]{};
\draw(4,-3) node[anchor=north]{}
--(4,-1) node[anchor=north]{};

\draw[-{Stealth[length=3mm]}](4,-5) node[anchor=north]{}
--(2,-4.5) node[anchor=north]{};
\draw(2,-4.5) node[anchor=north]{}
--(0,-4) node[anchor=north]{};

\draw[-{Stealth[length=3mm]}](6,2) node[anchor=north]{}
-- (5,0.5) node[anchor=north]{};
\draw(5,0.5) node[anchor=north]{}
-- (4,-1) node[anchor=north]{};

\draw[-{Stealth[length=3mm]}](6,2) node[anchor=north]{}
-- (4,2.5) node[anchor=north]{};
\draw(4,2.5) node[anchor=north]{}
-- (2,3) node[anchor=north]{};


\draw  [-{Stealth[length=3mm]}](0,-4) node[anchor=north]{}
--(0,-2) node[anchor=north]{};

\draw  [-{Stealth[length=3mm]}](-4,-1) node[anchor=south]{}
--(-2,-0.5) node[anchor=north]{};

\draw  [-{Stealth[length=3mm]}](-2,3) node[anchor=north]{}
--(-1,1.5) node[anchor=north]{};

\draw  [-{Stealth[length=3mm]}](2,3) node[anchor=north]{}
--(1,1.5) node[anchor=north]{};

\draw  [-{Stealth[length=3mm]}](4,-1) node[anchor=north]{}
--(2,-0.5) node[anchor=north]{};

\draw (0,-2) node[anchor=north]{}
--(0,0) node[anchor=north]{};

\draw (-2,-0.5) node[anchor=south]{}
--(0,0) node[anchor=north]{};

\draw (-1,1.5) node[anchor=north]{}
--(0,0) node[anchor=north]{};

\draw (1,1.5) node[anchor=north]{}
--(0,0) node[anchor=north]{};

\draw (2,-0.5) node[anchor=north]{}
--(0,0) node[anchor=north]{};


\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (6,2) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (4,-5) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-4,-5) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-6, 2) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (0,6) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (0,-4) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-4,-1) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (-2,3) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (2,3) {};
\node[circle,fill=black,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (4,-1) {};
\node[circle,fill=red,inner sep=0pt,minimum size=4pt,label=below:{}] (a) at (0,0) {};

\draw(0, 0.2) node[anchor=south]{$x$};

\end{tikzpicture}
\]
\end{figure}


==> Irrational_slope_section/Figures_code.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]

     \node [main node, draw=black] (x1) {\textit{$X_1$}};  
     \node [main node, draw=black] (x0)[right of=x1] {\textit{$X_0$}}; 
     \node [main node] (b)[right of=x0] {}; 
     \node [main node, draw=black] (a)[right of=b] {\textit{$\alpha$}}; 
     \node [main node] (y)[below of=x0] {}; 
     \node [main node, draw=black] (id)[below of=y] {\textit{$id$}};
     
     \path (x1) edge node {$0/0$} (id);
     \path (x1) edge  node {$1/1$} (x0);
     \path (x0) edge  node {$0/\epsilon$} (a);
     \path (x0) edge node {$1/11$} (id);
     \path (a) edge node [above] {$0/0$} (id);
     \path (a) edge [bend left] node {$1/10$} (id);
     \path (id) edge [out=170,in=140,looseness=12] node  {$0/0$} (id);
     \path (id) edge [out=220,in=190,looseness=12] node  {$1/1$} (id);

     \node [main node] (yy)[below of=id] {};
     \node [main node, draw=black] (y0)[below of=yy] {\textit{$Y_0$}};
     \node [main node, draw=black] (y1)[left of=y0] {\textit{$Y_1$}};
     \node [main node] (bb)[right of=y0] {\textit{}};
     \node [main node, draw=black] (b)[right of=bb] {\textit{$\beta$}};
     \node [main node, draw=black] (c)[above of=b] {\textit{$\gamma$}};

     \path (y1) edge node {$0/0$} (id);
     \path (y1) edge  node {$1/1$} (y0);
     \path (y0) edge  node {$0/\epsilon$} (b);
     \path (y0) edge  node [below right]{$1/11$} (id);
     \path (b) edge [loop right] node  {$0/0$} (b);
     \path (b) edge  node {$1/\epsilon$} (c);
     \path (c) edge  node {$0/011$} (id);
     \path (c) edge [bend right] node[above] {$1/10$} (id);

    \node [main node] (yyyyy)[left of=id] {};
    \node [main node] (yyyyyy)[left of=yyyyy] {};
     
\end{tikzpicture}

\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]     
     
     
     \node [main node, draw=black] (x0) {\textit{$C_1$}}; 
     \node [main node] (b)[right of=x0] {}; 
     \node [main node, draw=black] (a)[right of=b] {\textit{$\delta_1$}}; 
     \node [main node] (y)[below of=x0] {}; 
     \node [main node, draw=black] (id)[below of=y] {\textit{$id$}};
     
     \path (x0) edge  node {$1/\epsilon$} (a);
     \path (x0) edge node [above right]{$0/10$} (id);
     \path (a) edge node [right] {$0/11$} (id);
     \path (a) edge [bend left] node [right]{$1/0$} (id);
     \path (id) edge [out=310,in=280,looseness=12] node [below] {$0/0$} (id);
     \path (id) edge [out=80,in=50,looseness=12] node[above]  {$1/1$} (id);

     \node [main node] (yy)[below of=id] {};
     \node [main node, draw=black] (y0)[below of=yy] {\textit{$C_2$}};
     \node [main node] (bb)[right of=y0] {\textit{}};
     \node [main node, draw=black] (b)[right of=bb] {\textit{$\delta_2$}};
     \node [main node, draw=black] (c)[above of=b] {\textit{$\delta_3$}};

     \path (y0) edge  node {$1/\epsilon$} (b);
     \path (y0) edge  node [below left]{$0/10$} (id);
     \path (b) edge node  {$0/110$} (id);
     \path (b) edge  node {$1/\epsilon$} (c);
     \path (c) edge  node [right]{$0/111$} (id);
     \path (c) edge [bend right] node[above] {$1/0$} (id);

    \node [main node] (pi)[left of=id] {};
     \node [main node, draw=black] (pi1)[left of=pi] {\textit{$\Pi_0$}};
     \node [main node, draw=black] (de)[above of=pi1] {\textit{$\gamma$}};
     \path (pi1) edge  node [below]{$0/10$}(id);
     \path (pi1) edge  node {$1/\epsilon$} (de);
     \path (de) edge  node [below] {$0/0$} (id);
     \path (de) edge [bend left] node [above]{$1/11$} (id);

     \node [main node, draw=black] (pi2)[below of=pi1] {\textit{$\Pi_1$}};
     \path (pi2) edge  node [below]{$0/0$}(id);
     \path (pi2) edge  node {$1/1$} (pi1);
\end{tikzpicture}

\caption{Automata that generate the Thompson group $V_\tau$.}
    \label{fig:v_tau automaton}
\end{figure}


\begin{figure} 
    \centering
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[midway,left]{$LL$}}]
    [,edge label={node[midway,right]{$R$}}
        [,l*=2, ,edge label={node[midway,left]{$LL$}}
            [,edge label={node[midway,left]{$L$}}]
            [,l*=2,edge label={node[midway,right]{$RR$}}]
        ]
        [,edge label={node[midway,right]{$R$}}]
    ]
]
\end{forest}
\qquad
\begin{forest}
for tree={
    coordinate, calign=fixed edge angles, calign angle=25, edge=thick,
    {}
}
[
    [,l*=2,edge label={node[midway,left]{$0$}}]
    [,edge label={node[midway,right]{$1$}}
        [,l*=2, ,edge label={node[midway,left]{$0$}}
            [,edge label={node[midway,left]{}}]
            [,l*=2,edge label={node[midway,right]{$11$}}]
        ]
        [,edge label={node[midway,right]{$1$}}]
    ]
]
\end{forest}
    \caption{Carets of the $y_1$ generator addressed by pairs $L$'s,$R$'s and $0$'s, $1$'s }
    \label{fig: LR example}
\end{figure}

\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]
     \node [main node, draw=black] (x0) {\textit{$X_0$}}; 
     \node [main node] (b)[right of=x0] {}; 
     \node [main node, draw=black] (a)[right of=b] {\textit{$\alpha$}}; 
     \node [main node, draw=black] (id)[below of=x0] {\textit{$id$}};
     \path (x0) edge  node {$0/\epsilon$} (a);
     \path (x0) edge node {$1/11$} (id);
     \path (a) edge node [above] {$0/0$} (id);
     \path (a) edge [bend left] node {$1/10$} (id);
     \path (id) edge [loop left] node  {$0/0$} (id);
     \path (id) edge [loop below] node  {$1/1$} (id);
\end{tikzpicture}
    \caption{The $X_0$ generator}
    \label{fig:X_0 gen}
\end{figure}

\begin{figure}[htbp]
   \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]
     \node [main node] (x0) {$\{0,1\}^\omega$}; 
     \node [main node] (x1)[right of=x0] {}; 
     \node [main node] (x2)[right of=x1] {$\{0,1\}^\omega$};
     \node [main node] (x11)[right of=x2] {}; 
     \node [main node] (x22)[right of=x11] {$\{0,1\}^\omega$};
     
     \node [main node] (c0)[below of=x0] {};
     \node [main node] (c2)[below of=x2] {};
     \node [main node] (y0)[below of=c0] {$\CC_\tau$};
     \node [main node] (y2)[below of=c2] {$\CC_\tau$};
     \node [main node] (c22)[below of=x22] {};
     \node [main node] (y22)[below of=c22] {$\CC_\tau$};

     
     \path (x0) edge  node {$g_1$} (x2);
     \path (x2) edge  node {$g_2$} (x22);
     \path (x0) edge  node {$h$} (y0);
     \path (x2) edge  node {$h$} (y2);
     \path (x22) edge  node {$h$} (y22);
     \path (y0) edge  node {$\phi(g_1)$} (y2);
     \path (y2) edge  node {$\phi(g_2)$} (y22);
     \path (x0) edge [bend left] node {$g_2\cdot g_1$} (x22);
     \path (y0) edge [bend right] node {$\phi(g_2\cdot g_1)$} (y22);

\end{tikzpicture}
    \caption{A diagram representing the homomorphism of $\phi$}
    \label{fig: phi homomorphism}
\end{figure}

\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]


     \node [main node, draw=black] (id)[] {\textit{$id^{-1}$}};

     \node [main node] (yy)[below of=id] {};
     \node [main node, draw=black] (y0)[below of=yy] {\textit{$\beta^{-1}$}};
     \node [main node, draw=black] (y1)[left of=yy] {\textit{$t$}};
     \node [main node] (bb)[right of=y0] {\textit{}};
     \node [main node, draw=black] (b)[right of=bb] {\textit{$\beta$}};
     \node [main node, draw=black] (c)[above of=b] {\textit{$\gamma$}};

     \path (y1) edge node {$0/1$} (id);
     \path (y0) edge  node {$0/\epsilon$} (b);
     \path (y0) edge node [right]{$1/ 1$} (y1);
     \path (b) edge [loop right] node  {$0/0$} (b);
     \path (b) edge  node {$1/\epsilon$} (c);
     \path (c) edge  node [below left, pos=0.2]{$0/011$} (id);
     \path (c) edge [bend right] node[above] {$1/10$} (id);
     \path (id) edge [out=170,in=140,looseness=12] node  {$0/0$} (id);
     \path (id) edge [out=110,in=80,looseness=12] node  {$1/1$} (id);

     \node [main node, draw=black] (ga)[below of=y1] {\textit{$\gamma^{-1}$}};
     \node [main node, draw=black] (u)[left of=ga] {\textit{$u$}};
     \node [main node, draw=black] (v)[left of=y1] {\textit{$v$}};

     \path (ga) edge  node {$1/\epsilon$} (y1);
     \path (ga) edge  node {$0/0$} (u);
     \path (u) edge  node {$1/\epsilon$} (v);
     \path (v) edge [bend left] node[above] {$1/\epsilon$} (id);
\end{tikzpicture}

\caption{Automata of the the inverse maps of $\beta$, $\gamma$ and $id$ of the Thompson group $V_\tau$}

    \label{fig:beta inverse automaton}
\end{figure}

\begin{figure}
    \centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]
     \node [main node, draw=black] (id)[] {\textit{$id$}};
     \node [main node] (g1)[left of =id] {};
     \node [main node, draw=black] (g)[above left of =g1] {\textit{$\gamma^2$}};
     \node [main node] (b1)[right of =id] {};
     \node [main node] (b2)[right of =b1] {};
     \node [main node, draw=black] (b)[above of =b2] {\textit{$\beta^2$}};  
    \node [main node] (gb)[above of =id] {};
     \node [main node, draw=black] (gb)[above of =gb] {\textit{$\gamma \beta$}};
     \node [main node] (bg1)[below of =id] {};
     \node [main node, draw=black] (bg)[below left of =bg1] {\textit{$\beta\gamma$}};

     \node [main node, draw=black] (beta)[below of =b2] {\textit{$\beta$}};
     \node [main node, draw=black] (gamma)[below of =beta] {\textit{$\gamma$}};     

     
     \path (b) edge [bend left] node [above,pos=0.6]{$1/1$} (id);
     \path (b) edge [bend right] node [below, pos=0.3]{$0/0$} (id);
     \path (g) edge [bend left] node [left,pos=0.6]{$1/1$} (id);
     \path (g) edge [bend right] node [below, pos=0.6]{$0/0$} (id);
     \path (gb) edge [bend left] node [right,pos=0.3]{$1/1$} (id);
     \path (gb) edge [bend right] node [right]{$0/0$} (id);
     \path (bg) edge [bend left] node [left, pos=0.4]{$1/1$} (id);
     \path (bg) edge [bend right] node[right] {$0/0$} (id);
     \path (id) edge [loop above] node  {$0/0$} (id);
     \path (id) edge [out=260,in=230,looseness=8] node [below] {$1/1$} (id);
     \path (gamma) edge [loop right] node  {$0/0$} (gamma);
     \path (gamma) edge [] node  {$1/\epsilon$} (beta);
     \path (beta) edge [bend right] node  {$1/10$} (id);
     \path (beta) edge [bend left] node [right,pos=0.5]  {$0/011$} (id);
\end{tikzpicture}
    \caption{The composition of states of $\NN$ }
    \label{fig:gamma square}
\end{figure}



\begin{figure}
    \centerline{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]
     \node [main node] (x0) {$\{0,1\}^\omega$}; 
     \node [main node] (x1)[right of=x0] {}; 
     \node [main node] (x2)[below right of=x1] {$\CC_\tau$};
     
     \node [main node] (c0)[below of=x0] {};
     \node [main node] (y0)[below of=c0] {$[0,1]$};
     
     \path (x0) edge  node {$h$} (x2);
     \path (x0) edge  node {$q$} (y0);
     \path (x2) edge  node {$\pi$} (y0);
\end{tikzpicture}
}   
\end{figure}


\begin{figure}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]
     \node [main node] (x0) {$\{0,1\}^\omega$}; 
     \node [main node] (x1)[right of=x0] {}; 
     \node [main node] (x2)[right of=x1] {$\{0,1\}^\omega$}; 
     \node [main node] (c0)[below of=x0] {};
     \node [main node] (c2)[below of=x2] {};
     \node [main node] (y0)[below of=c0] {$\{0,1\}^\omega$};
     \node [main node] (y2)[below of=c2] {$\{0,1\}^\omega$};     
     \node [main node] (d0)[below of=y0] {};
     \node [main node] (d2)[below of=y2] {};
     \node [main node] (z0)[below of=d0] {$[0,1]$};
     \node [main node] (z2)[below of=d2] {$[0,1]$};     
     
     \path (x0) edge  node {$X_0$} (x2);
     \path (x0) edge  node {$q_1$} (y0);
     \path (x2) edge  node {$q_1$} (y2);
     \path (y0) edge  node {$q_2$} (z0);
     \path (y2) edge  node {$q_2$} (z2);
     \path (z0) edge  node {$x_0$} (z2);
     \path (x0) edge [bend right] node {$q$} (z0);
     \path (x2) edge [bend left] node {$q$} (z2);
\end{tikzpicture}
\end{figure}


\begin{figure}
    \centerline{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm, thick,main node/.style={circle,font=\bfseries}]
     \node [main node] (x0) {$\{0,1\}^\omega$}; 
     \node [main node] (x1)[right of=x0] {}; 
     \node [main node] (x2)[right of=x1] {$\{0,1\}^\omega$};
     
     \node [main node] (c0)[below of=x0] {};
     \node [main node] (c2)[below of=x2] {};
     \node [main node] (y0)[below of=c0] {$\CC_\tau$};
     \node [main node] (y2)[below of=c2] {$\CC_\tau$};
     
     \path (x0) edge  node {$g$} (x2);
     \path (x0) edge  node {$h$} (y0);
     \path (x2) edge  node {$h$} (y2);
     \path (y0) edge  node {$\phi(g)$} (y2);

\end{tikzpicture}
}  
\end{figure}
